Knowledge Graph-enhanced Sampling for Conversational Recommender System

The traditional recommendation systems mainly use offline user data to train offline models, and then recommend items for online users, thus suffering from the unreliable estimation of user preferences based on sparse and noisy historical data. Conversational Recommendation System (CRS) uses the interactive form of the dialogue systems to solve the intrinsic problems of traditional recommendation systems. However, due to the lack of contextual information modeling, the existing CRS models are unable to deal with the exploitation and exploration (E&E) problem well, resulting in the heavy burden on users. To address the aforementioned issue, this work proposes a contextual information enhancement model tailored for CRS, called Knowledge Graph-enhanced Sampling (KGenSam). KGenSam integrates the dynamic graph of user interaction data with the external knowledge into one heterogeneous Knowledge Graph (KG) as the contextual information environment. Then, two samplers are designed to enhance knowledge by sampling fuzzy samples with high uncertainty for obtaining user preferences and reliable negative samples for updating recommender to achieve efficient acquisition of user preferences and model updating, and thus provide a powerful solution for CRS to deal with E&E problem. Experimental results on two real-world datasets demonstrate the superiority of KGenSam with significant improvements over state-of-the-art methods.

==> sketch.tex <==


目前的研究工作无法为EE问题提供一个有效的解决方案，这导致了crs无法高效且准确的进行交互推荐。
我们相信ee问题解决的欠缺很大程度上是因为CRS没有很好的利用交互环境的信息，CRS框架中缺乏对环境信息的充分建模。因此我们从数据增强的角度出发，引入知识图谱作为环境，设计两个采样器去增强图谱环境的信息，帮助CRS基于增强的知识去做EE的决策，实现高效的用户偏好获取和有限轮次内准确的推荐。

KGenSam采取在KG中采样的方式，增强知识，我们设计KGenSam中两个采样器的启发在于解决以下两个困扰CRS去做出最优EE决策的具体问题：
CRS询问什么物品属性能最大程度地去帮助推荐器去拟合当前用户的偏好？
CRS如何最快速地更新推荐器去拟合当前用户的反馈信息？


该研究框架的工作流程如下：
（1）首先，我们构建用户交互行为的知识图谱，并融合外部知识图谱，丰富交互环境的上下文信息，用知识辅助CRS交互智能体进行交互决策。
（2）在知识图谱的环境基础上，我们设计了两个基于强化学习的采样器，在知识图谱中分别去采样模糊样本和负样本，增强了知识。具体来说，一是，主动采样器关注于图中代表用户偏好的属性样本节点，通过主动强化学习去输出具有较大不确定性的模糊样本，模糊样本用于交互中的询问动作，高效提高模型置信度，从而提高系统的交互效率；二是，负采样器关注于图中的物品样本节点，通过强化学习输出高质量的负样本，负样本去补充稀疏的线上用户数据，高效更新推荐器，从而提高推荐模型的更新效率。两部分共同发挥作用，实现用户偏好的高效获取，并减少交互轮次，也就能减轻用户交互负担。
（3）最后，我们设计一个简单的CRS交互强化策略网络，在两个采样器的帮助下，交互策略网络基于增强的知识去学习交互策略，策略网络输出系统将要采取的动作（询问或推荐），引导用户的交互，实现在线用户偏好的获取与契合用户当前偏好的物品推荐。



当解决了crs询问什么属性使每轮ask机会的效率最高的问题后，另一个问题自然而然的需要被考虑到，即用户对于模糊样本的反馈信号如何能被推荐器准确学习到？考虑到对话推荐一次会话的时间较短，推荐器的学习速度需要又准又快。

